Temporal Alignment Networks for Long-term Video

The objective of this paper is a temporal alignment network that ingests long term video sequences, and associated text sentences, in order to: (1) determine if a sentence is alignable with the video; and (2) if it is alignable, then determine its alignment. The challenge is to train such networks from large-scale datasets, such as HowTo100M, where the associated text sentences have significant noise, and are only weakly aligned when relevant. Apart from proposing the alignment network, we also make four contributions: (i) we describe a novel co-training method that enables to denoise and train on raw instructional videos without using manual annotation, despite the considerable noise; (ii) to benchmark the alignment performance, we manually curate a 10-hour subset of HowTo100M, totalling 80 videos, with sparse temporal descriptions. Our proposed model, trained on HowTo100M, outperforms strong baselines (CLIP, MIL-NCE) on this alignment dataset by a significant margin; (iii) we apply the trained model in the zero-shot settings to multiple downstream video understanding tasks and achieve state-of-the-art results, including text-video retrieval on YouCook2, and weakly supervised video action segmentation on Breakfast-Action; (iv) we use the automatically aligned HowTo100M annotations for end-to-end finetuning of the backbone model, and obtain improved performance on downstream action recognition tasks.

==> backup.tex <==

\maketitle

\input{sec/01-abstract}
\input{sec/02-introduction}
\input{sec/03-related_work}
\input{sec/04-method}
\input{sec/05-experiment}
\input{sec/06-downstream}
\input{sec/07-conclusion}


==> sec/teaser.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{figure*}[H]
    \centering
    \includegraphics[width=\textwidth]{img/align3.pdf}
    \vspace*{-8mm}
    \captionof{figure}{
	\footnotesize{An example of visual-textual mis-alignment in a raw instructional video.
	The presenter's narration can be visually not relevant at all, {\em e.g.}~describing flavor;
	or asynchronous with visual content by a time difference.
	The \textcolor{googleblue}{\textbf{\cmark}} and \textcolor{googleorange}{\textbf{\xmark}} 
	indicate visually alignable and non-alignable text respectively (by human judgement). 
	The colored bar shows the start-end timestamp of narration. 
	Example from \scriptsize{\url{https://www.youtube.com/watch?v=M8OGXmLTTiI?t=30}}.}}
\end{figure*}%
}]


\begin{comment}
%%%%%%%%%%%%%%%%%%%
% teaser figure %%%
\begin{figure*}[t]
    \centering
	\includegraphics[width=\textwidth]{img/align3.pdf}
	\vspace*{-8mm}
	\caption{
	\footnotesize{An example of visual-textual mis-alignment in a raw instructional video.
	The presenter's narration can be visually not relevant at all, {\em e.g.}~describing flavor;
	or asynchronous with visual content by a time difference.
	The \textcolor{googleblue}{\textbf{\cmark}} and \textcolor{googleorange}{\textbf{\xmark}} 
	indicate visually alignable and non-alignable text respectively (by human judgement). 
	The colored bar shows the start-end timestamp of narration. 
	Example from \scriptsize{\url{https://www.youtube.com/watch?v=M8OGXmLTTiI?t=30}}.}}
\vspace{-15pt}
\label{fig:align}
\end{figure*}
%%%%%%%%%%%%%%%%%%%
\end{comment}
